DataEvolver: Let Your Data Build and Improve Itself via Goal-Driven Loop Agents

Constructing controllable visual data is a major bottleneck for image editing and multimodal understanding. Useful supervision is rarely produced by a single rendering pass; instead it emerges through iterative generation, inspection, correction, filtering, and export. We present DataEvolver, a closed-loop visual data engine that organizes this process around explicit goals, persistent artifacts, bounded corrective actions, and acceptance decisions. DataEvolver supports multiple artifact types, including RGB images, masks, depth maps, normal maps, meshes, poses, trajectories, and review traces. In the current release, the system operates through two coupled loops: generation-time self-correction within each sample and validation-time self-expansion across dataset rounds. We validate the framework on an image-level object-rotation setting. With a fixed Qwen-Edit LoRA probe, our final Ours+DualGate model outperforms both the unadapted base model and a public multi-angle LoRA on SpatialEdit and a held-out evaluation set. Ablations show a consistent improvement path from scene-aware generation to feedback-driven correction and dual-gated validation. Beyond the released rotation data, our main contribution is a reusable framework for building visual datasets through explicit goal tracking, review, correction, and acceptance loops.

==> unused_tables/generated/ablation_design_booktabs.tex <==
% Auto-generated by scripts/generate_feedback_ablation_assets.py
\begin{tabular}{llllr}
\toprule
Condition & Outer feedback & Inner gate & Post gate & Train pairs \\
\midrule
No feedback loop & No & No & No & 245 \\
Outer loop only & Yes & No & No & 305 \\
Outer + inner gate & Yes & Yes & No & 473 \\
Outer + inner + post gate & Yes & Yes & Yes & 325 \\
\bottomrule
\end{tabular}


==> unused_tables/generated/ablation_metrics_booktabs.tex <==
% Auto-generated by scripts/generate_feedback_ablation_assets.py
\begin{tabular}{lrr}
\toprule
Condition & Score\_view & VIE Overall \\
\midrule
No feedback loop & 0.7705 & 0.8649 \\
Outer loop only & \textbf{0.7828} & 0.8703 \\
Outer + inner gate & \textbf{0.7828} & \textbf{0.8753} \\
Outer + inner + post gate & \textbf{0.7828} & \textbf{0.8753} \\
\bottomrule
\end{tabular}


==> unused_tables/generated/dataset_stats_booktabs.tex <==
% Updated from eval_results/ablation_chain_summary.csv and ablation-chain notes.
\begin{tabular}{lrrrrl}
\toprule
Configuration & Train objects & Train pairs & Val pairs & Test pairs & Intervention \\
\midrule
Ours-Base & 35 & 245 & 49 & 56 & no external feedback loop \\
Ours +Feedback & 35+20 & 305 & 49 & 56 & outer-loop weak-angle feedback, no gate \\
Ours +InnerGate & -- & 473 & 49 & 56 & outer loop with internal render-quality gate \\
Ours +DualGate & -- & 325 & 49 & 56 & internal gate plus external post-feedback gate \\
\bottomrule
\end{tabular}


==> unused_tables/generated/full_gate_spatialedit_per_angle_booktabs.tex <==
% Auto-generated by scripts/generate_feedback_ablation_assets.py
\begin{tabular}{rrrrrrrr}
\toprule
Angle & Supp. & PSNR & SSIM & LPIPS & CLIP-I & Score\_view & VIE \\
\midrule
0 & no & 17.09 & 0.735 & 0.250 & 0.955 & 0.9508 & 0.9689 \\
45 & no & 16.44 & 0.723 & 0.266 & 0.956 & 0.6230 & 0.7852 \\
90 & no & 17.81 & 0.758 & 0.199 & 0.957 & 0.9508 & 0.9672 \\
135 & yes & 16.33 & 0.725 & 0.262 & 0.955 & 0.5738 & 0.7664 \\
180 & no & 17.19 & 0.736 & 0.246 & 0.958 & 0.8197 & 0.9000 \\
225 & yes & 15.76 & 0.721 & 0.280 & 0.941 & 0.7541 & 0.8516 \\
270 & yes & 16.65 & 0.744 & 0.251 & 0.934 & 0.8689 & 0.9238 \\
315 & yes & 16.35 & 0.727 & 0.271 & 0.946 & 0.7213 & 0.8393 \\
\bottomrule
\end{tabular}


==> unused_tables/generated/full_gate_testset_summary_booktabs.tex <==
% Auto-generated by scripts/generate_feedback_ablation_assets.py
\begin{tabular}{lrrrr}
\toprule
Split & PSNR & SSIM & LPIPS & CLIP-I \\
\midrule
SpatialEdit-Bench & 16.70 & 0.7336 & 0.2531 & 0.9503 \\
In-domain testset & 28.95 & 0.9176 & 0.0855 & 0.9640 \\
\bottomrule
\end{tabular}


==> unused_tables/generated/indomain_sanity_comparison_booktabs.tex <==
% In-domain 56-pair sanity check from the experiment record.
\begin{tabular}{lrrrr}
\toprule
Probe & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & CLIP-I $\uparrow$ \\
\midrule
Base model & 22.51 & 0.7859 & 0.2451 & 0.9253 \\
Public multi-angle LoRA & 12.49 & 0.5133 & 0.5701 & 0.8996 \\
\bottomrule
\end{tabular}


==> unused_tables/generated/overall_metrics_booktabs.tex <==
% Auto-generated by arxiv_report/paper/scripts/generate_latex_assets.py
\begin{tabular}{lrrrl}
\toprule
Metric & Semantic baseline & Feedback R1 & $\Delta$ & Interpretation \\
\midrule
PSNR ($\uparrow$) & 16.63 & 16.68 & +0.05 & better \\
SSIM ($\uparrow$) & 0.7296 & 0.731 & +0.0014 & better \\
LPIPS ($\downarrow$) & 0.2564 & 0.2546 & -0.0018 & better \\
CLIP-I ($\uparrow$) & 0.905 & 0.9499 & +0.0449 & better \\
Score\_view ($\uparrow$) & 0.7705 & 0.7828 & +0.0123 & better \\
\bottomrule
\end{tabular}


==> unused_tables/generated/per_angle_diagnostics_booktabs.tex <==
% Auto-generated by arxiv_report/paper/scripts/generate_latex_assets.py
\begin{tabular}{rrrrr}
\toprule
Angle & Score\_view Semantic & Score\_view R1 & $\Delta$ & PSNR $\Delta$ \\
\midrule
45 & 0.9344 & 0.9508 & +0.0160 & +0.0200 \\
90 & 0.6066 & 0.5738 & -0.0330 & +0.0600 \\
135 & 1.0000 & 1.0000 & +0.0000 & +0.1300 \\
180 & 0.5574 & 0.6066 & +0.0490 & +0.0300 \\
225 & 0.8197 & 0.8689 & +0.0490 & +0.2200 \\
270 & 0.7541 & 0.7541 & +0.0000 & +0.0600 \\
315 & 0.9016 & 0.8852 & -0.0160 & -0.0200 \\
360 & 0.5902 & 0.6230 & +0.0330 & -0.0700 \\
\bottomrule
\end{tabular}


==> unused_tables/generated/r1_augmentation_composition_booktabs.tex <==
% Auto-generated by arxiv_report/paper/scripts/generate_latex_assets.py
\begin{tabular}{lrl}
\toprule
Group & Count & Unit \\
\midrule
daily\_item & 10 & objects \\
sports\_item & 3 & objects \\
street\_object & 4 & objects \\
vehicle & 3 & objects \\
target yaw 90$^\circ$ & 20 & pairs \\
target yaw 180$^\circ$ & 20 & pairs \\
target yaw 270$^\circ$ & 20 & pairs \\
\bottomrule
\end{tabular}


==> unused_tables/generated/r1_quality_diagnosis_booktabs.tex <==
% Auto-generated by arxiv_report/paper/scripts/generate_latex_assets.py
\begin{tabular}{ll}
\toprule
Diagnostic item & Value \\
\midrule
New feedback-scaling objects & 20 \\
Objects below hybrid-score gate 0.6 & 20 \\
Median latest hybrid score & 0.447 \\
Min / max latest hybrid score & 0.365 / 0.582 \\
Verdict & inspect \\
Next action & render-quality gating before merge \\
\bottomrule
\end{tabular}


==> unused_tables/generated/r2_gate_comparison_booktabs.tex <==
% Auto-generated by scripts/generate_r2_latex_assets.py
\begin{tabular}{lccc}
\toprule
Round & New objects & Render-quality gate & Training pairs \\
\midrule
exp5 baseline & 0 & none & 245 \\
R1 & 20 & post-hoc diagnosis only & 305 \\
R2 & 20 & internal gate $\geq 0.5$ & 473 \\
\bottomrule
\end{tabular}


==> unused_tables/generated/r2_spatialedit_per_angle_booktabs.tex <==
% Auto-generated by scripts/generate_r2_latex_assets.py
\begin{tabular}{rrrrrr}
\toprule
Angle & PSNR & SSIM & LPIPS & CLIP-I & DINO \\
\midrule
0 & 17.32 & 0.741 & 0.241 & 0.958 & 0.905 \\
45 & 16.57 & 0.732 & 0.259 & 0.954 & 0.906 \\
90 & 18.02 & 0.763 & 0.196 & 0.956 & 0.913 \\
135 & 16.34 & 0.729 & 0.261 & 0.959 & 0.898 \\
180 & 17.18 & 0.738 & 0.245 & 0.958 & 0.909 \\
225 & 15.68 & 0.721 & 0.281 & 0.946 & 0.859 \\
270 & 16.44 & 0.743 & 0.255 & 0.928 & 0.841 \\
315 & 16.41 & 0.733 & 0.264 & 0.948 & 0.888 \\
\bottomrule
\end{tabular}


==> unused_tables/generated/r2_spatialedit_traditional_booktabs.tex <==
% Auto-generated by scripts/generate_r2_latex_assets.py
\begin{tabular}{lrrrrr}
\toprule
Metric & exp5 & R1 & R2 & R2--exp5 & R2--R1 \\
\midrule
PSNR ($\uparrow$) & 16.63 & 16.68 & 16.74 & +0.1143 & +0.0643 \\
SSIM ($\uparrow$) & 0.7296 & 0.7310 & 0.7376 & +0.0080 & +0.0066 \\
LPIPS ($\downarrow$) & 0.2564 & 0.2546 & 0.2501 & -0.0063 & -0.0045 \\
CLIP-I ($\uparrow$) & 0.9050 & 0.9499 & 0.9509 & +0.0459 & +0.0010 \\
DINO ($\uparrow$) & 0.8895 & 0.8837 & 0.8898 & +0.0003 & +0.0061 \\
\bottomrule
\end{tabular}


==> unused_tables/generated/r2_testset_summary_booktabs.tex <==
% Auto-generated by scripts/generate_r2_latex_assets.py
\begin{tabular}{lrrr}
\toprule
Split / benchmark & Pairs & PSNR & SSIM / LPIPS \\
\midrule
SpatialEdit-Bench & 488 & 16.74 & 0.7376 / 0.2501 \\
In-domain testset & 56 & 31.48 & 0.9425 / 0.0382 \\
\bottomrule
\end{tabular}


==> unused_tables/generated/r2_viescore_booktabs.tex <==
% Auto-generated by scripts/generate_r2_latex_assets.py
\begin{tabular}{lrrrrr}
\toprule
Metric & exp5 & R1 & R2 & R2--exp5 & R2--R1 \\
\midrule
Score\_view ($\uparrow$) & 0.7705 & 0.7828 & 0.7828 & +0.0123 & +0.0000 \\
Score\_cons ($\uparrow$) & 0.9709 & 0.9676 & 0.9678 & -0.0031 & +0.0002 \\
VIE Overall ($\uparrow$) & 0.8649 & 0.8703 & 0.8753 & +0.0104 & +0.0050 \\
\bottomrule
\end{tabular}


==> unused_tables/generated/r3_spatialedit_per_angle_booktabs.tex <==
% Auto-generated by scripts/generate_feedback_ablation_assets.py
\begin{tabular}{rrrrrrrr}
\toprule
Angle & Supp. & PSNR & SSIM & LPIPS & CLIP-I & Score\_view & VIE \\
\midrule
0 & no & 17.09 & 0.735 & 0.250 & 0.955 & 0.9508 & 0.9689 \\
45 & no & 16.44 & 0.723 & 0.266 & 0.956 & 0.6230 & 0.7852 \\
90 & no & 17.81 & 0.758 & 0.199 & 0.957 & 0.9508 & 0.9672 \\
135 & yes & 16.33 & 0.725 & 0.262 & 0.955 & 0.5738 & 0.7664 \\
180 & no & 17.19 & 0.736 & 0.246 & 0.958 & 0.8197 & 0.9000 \\
225 & yes & 15.76 & 0.721 & 0.280 & 0.941 & 0.7541 & 0.8516 \\
270 & yes & 16.65 & 0.744 & 0.251 & 0.934 & 0.8689 & 0.9238 \\
315 & yes & 16.35 & 0.727 & 0.271 & 0.946 & 0.7213 & 0.8393 \\
\bottomrule
\end{tabular}


==> unused_tables/generated/r3_supplemented_angles_booktabs.tex <==
% Auto-generated by scripts/generate_feedback_ablation_assets.py
\begin{tabular}{rrrrrrrrrr}
\toprule
Angle & PSNR exp5 & PSNR R1 & PSNR R3 & $\Delta$ & View exp5 & View R1 & View R3 & $\Delta$ & Verdict \\
\midrule
135 & 16.08 & 16.12 & 16.33 & +0.25 & 0.5574 & 0.6066 & 0.5738 & +0.0164 & gain \\
225 & 15.73 & 15.78 & 15.76 & +0.03 & 0.7541 & 0.7541 & 0.7541 & +0.0000 & gain \\
270 & 16.64 & 16.62 & 16.65 & +0.01 & 0.9016 & 0.8852 & 0.8689 & -0.0327 & mixed \\
315 & 16.33 & 16.26 & 16.35 & +0.02 & 0.5902 & 0.6230 & 0.7213 & +0.1311 & gain \\
\bottomrule
\end{tabular}


==> unused_tables/generated/r3_testset_summary_booktabs.tex <==
% Auto-generated by scripts/generate_feedback_ablation_assets.py
\begin{tabular}{lrrrr}
\toprule
Split & PSNR & SSIM & LPIPS & CLIP-I \\
\midrule
SpatialEdit-Bench & 16.70 & 0.7336 & 0.2531 & 0.9503 \\
In-domain testset & 28.95 & 0.9176 & 0.0855 & 0.9640 \\
\bottomrule
\end{tabular}


==> unused_tables/generated/spatialedit_comparison_booktabs.tex <==
% External comparison using final Ours +DualGate as Ours.
\begin{tabular}{lrrrrr}
\toprule
Method & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & CLIP-I $\uparrow$ & DINO $\uparrow$ \\
\midrule
Base (Qwen-Image-Edit-2511) & 14.97 & 0.6455 & 0.3625 & 0.8780 & 0.7832 \\
Public LoRA & 15.76 & 0.6545 & 0.3443 & 0.8900 & 0.8444 \\
Ours +DualGate & \textbf{16.79} & \textbf{0.7395} & \textbf{0.2478} & \textbf{0.9525} & \textbf{0.8918} \\
\bottomrule
\end{tabular}


==> unused_tables/generated/targeted_angles_booktabs.tex <==
% Auto-generated by scripts/generate_feedback_ablation_assets.py
\begin{tabular}{rrrrrrrrrrr}
\toprule
Angle & PSNR no loop & PSNR outer & PSNR inner & PSNR post & $\Delta$ & View no loop & View outer & View post & $\Delta$ & Verdict \\
\midrule
135 & 16.08 & 16.12 & 16.34 & 16.33 & +0.25 & 0.5574 & 0.6066 & 0.5738 & +0.0164 & gain \\
225 & 15.73 & 15.78 & 15.68 & 15.76 & +0.03 & 0.7541 & 0.7541 & 0.7541 & +0.0000 & gain \\
270 & 16.64 & 16.62 & 16.44 & 16.65 & +0.01 & 0.9016 & 0.8852 & 0.8689 & -0.0327 & mixed \\
315 & 16.33 & 16.26 & 16.41 & 16.35 & +0.02 & 0.5902 & 0.6230 & 0.7213 & +0.1311 & gain \\
\bottomrule
\end{tabular}


==> unused_tables/generated/v4_spatialedit_table.tex <==
\begin{table}[t]
\centering
\caption{External model comparison on SpatialEdit-Bench (488 pairs). Ours uses the final DualGate model.}
\label{tab:external_spatialedit}
% External comparison using final Ours +DualGate as Ours.
\begin{tabular}{lrrrrr}
\toprule
Method & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & CLIP-I $\uparrow$ & DINO $\uparrow$ \\
\midrule
Base (Qwen-Image-Edit-2511) & 14.97 & 0.6455 & 0.3625 & 0.8780 & 0.7832 \\
Public LoRA & 15.76 & 0.6545 & 0.3443 & 0.8900 & 0.8444 \\
Ours & \textbf{16.79} & \textbf{0.7395} & \textbf{0.2478} & \textbf{0.9525} & \textbf{0.8918} \\
\bottomrule
\end{tabular}
\end{table}


==> unused_tables/generated/v4_testset_comparison_booktabs.tex <==
% External comparison using final Ours +DualGate as Ours.
\begin{tabular}{lrrrrr}
\toprule
Method & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & CLIP-I $\uparrow$ & DINO $\uparrow$ \\
\midrule
Base (Qwen-Image-Edit-2511) & 14.92 & 0.7179 & 0.3145 & 0.9127 & 0.8787 \\
Public LoRA & 15.20 & 0.7550 & 0.2750 & 0.9300 & 0.8950 \\
Ours +DualGate & \textbf{28.95} & \textbf{0.9176} & \textbf{0.0855} & \textbf{0.9640} & \textbf{0.9282} \\
\bottomrule
\end{tabular}


==> unused_tables/generated/v4_testset_table.tex <==
\begin{table}[t]
\centering
\caption{External model comparison on Eval1 Test Set (56 pairs). Ours uses the final DualGate model.}
\label{tab:external_testset}
% External comparison using final Ours +DualGate as Ours.
\begin{tabular}{lrrrrr}
\toprule
Method & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & CLIP-I $\uparrow$ & DINO $\uparrow$ \\
\midrule
Base (Qwen-Image-Edit-2511) & 14.92 & 0.7179 & 0.3145 & 0.9127 & 0.8787 \\
Public LoRA & 15.20 & 0.7550 & 0.2750 & 0.9300 & 0.8950 \\
Ours & \textbf{28.95} & \textbf{0.9176} & \textbf{0.0855} & \textbf{0.9640} & \textbf{0.9282} \\
\bottomrule
\end{tabular}
\end{table}


==> unused_tables/generated/vlm_score_comparison_booktabs.tex <==
% VLM judge comparison from experiment logs and current exp5/R1 VIEScore CSV-derived reports.
\begin{tabular}{lr}
\toprule
Probe & Score\_view $\uparrow$ \\
\midrule
Base model & 0.7746 \\
Public multi-angle LoRA & 0.7234 \\
Semantic-Object Prompt LoRA & 0.7705 \\
Feedback-Guided Scaling R1 & \textbf{0.7828} \\
\bottomrule
\end{tabular}

